Embed and Emulate: Contrastive representations for simulation-based inference

Scientific modeling and engineering applications rely heavily on parameter estimation methods to fit physical models and calibrate numerical simulations using real-world measurements. In the absence of analytic statistical models with tractable likelihoods, modern simulation-based inference (SBI) methods first use a numerical simulator to generate a dataset of parameters and simulated outputs. This dataset is then used to approximate the likelihood and estimate the system parameters given observation data. Several SBI methods employ machine learning emulators to accelerate data generation and parameter estimation. However, applying these approaches to high-dimensional physical systems remains challenging due to the cost and complexity of training high-dimensional emulators. This paper introduces Embed and Emulate (E&E): a new SBI method based on contrastive learning that efficiently handles high-dimensional data and complex, multimodal parameter posteriors. E&E learns a low-dimensional latent embedding of the data (i.e., a summary statistic) and a corresponding fast emulator in the latent space, eliminating the need to run expensive simulations or a high dimensional emulator during inference. We illustrate the theoretical properties of the learned latent space through a synthetic experiment and demonstrate superior performance over existing methods in a realistic, non-identifiable parameter estimation task using the high-dimensional, chaotic Lorenz 96 system.

==> imgs/plot_12.tex <==
\begin{figure}[t]
\centering
\begin{minipage}{1\textwidth}
  \centering
  \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[trim={0.3cm 0.5cm 7cm 6.6cm},clip,height=4.5cm]{figures/ours_102.pdf}
    \caption{\eande}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[trim={0.3cm 0.5cm 7cm 6.6cm},clip,height=4.5cm]{figures/nre_102.pdf}
    \caption{NRE-C}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.37\textwidth}
    \centering
    \includegraphics[trim={0.3cm 0.5cm 3cm 6.6cm},clip, height=4.5cm]{figures/npe_102.pdf}
    \caption{NPE-C}
  \end{subfigure}
\end{minipage}
\caption{\textbf{Visual comparison of the estimated joint and marginal posterior distributions for one test sample.} 
% In each subplot, the dashed red line in the bottom left section indicates the ground truth reference distribution, represented as the red dashed circle, while the heatmap displays the estimated posterior probabilities.
% The histograms showing marginal densities in the upper and right portions of each subplot are plotted using samples drawn from the estimated posterior using the acceptance-rejection sampling, with the dashed black line illustrating the histograms of samples from the reference distribution.
The results illustrate that \eande captures the full spread of the posterior, whereas NRE-C \citep{miller2022contrastive} and NPE-C \citep{greenberg2019automatic} concentrate on limited regions of the circle, resulting in skewed estimates.
}
\label{fig:posterior_12}
\end{figure}


==> tables/table_l96.tex <==
\begin{table}[t]
\scalebox{0.9}{
\centering
\begin{tabular}{p{9em}p{16em}p{16em}}
\toprule
Method & {MMD ($\sigma = 0.01$) $\downarrow$} & {MMD ($\sigma = 0.05$) $\downarrow$} \\
\midrule
\sc{NPE-C} & 1.509e-03(1.439e-03, 1.797e-03) & 1.713e-03(1.527e-03, 3.578e-03)
\\
\midrule
\sc{NRE-C} & 1.509e-03(1.439e-03, 1.797e-03) & 1.713e-03(1.527e-03, 3.578e-03)
\\
\midrule
\eande & \textbf{1.226e-03(1.023e-03, 1.559e-03)} & \textbf{6.617e-04(3.986e-04, 1.170e-03)}
\\
\bottomrule
\end{tabular}}
\caption{\textbf{Empirical performance showing for 50 test samples.} The median(25th, 75th percentile) of the Maximum mean discrepancy (MMD) is presented for kernel scales $\sigma = 0.01$ and $\sigma = 0.05$. For each test instance, we draw two sets of 5,000 samples from (1) the estimated $\hat{q}(\bphi|\by^o)$ with rejection sampling; and (2) the true $p(\bphi|y^o)$. The MMD is then calculated between these two sets of samples.
We show significant improvements of \eande, evidenced by a decrease in the values and spread of error statistics.} 
\label{table:multimodal_eval}
\end{table}

